Prospects for Slepton Searches in Future Experiments

Muon g-2 anomaly, which is mismatch between the theoretical and the experimental values of the anomalous magnetic moment of muons, provides a sensitive probe of new physics. In SUSY, if masses of the superpartners relevant to the muon g-2 are O(100) GeV, the SUSY contributions to the muon g-2 become sizable and the anomaly can be solved. There are two representative SUSY contributions to the muon g-2, the chargino and the neutralino contributions, respectively. Particularly, when the discrepancy of the muon g-2 is dominated by the neutralino contributions, it is found that the discrepancy can be explained if only the Bino and sleptons are light. This setup is "minimal" to solve the muon g-2 anomaly. In this dissertation, we discuss the "minimal" SUSY models where only the Bino and sleptons are light, while the other superparticles are decoupled. When the slepton soft masses are universal, we show that the upper bound on the smuon mass becomes 330 (460) GeV in order to solve the muon g-2 anomaly at the 1sigma (2 sigma) level. It is within the reach of LHC and ILC. Further, light staus might affect the Higgs coupling to di-photon, which is sensitive to new physics. We also study future prospects of the stau which contributes to the Higgs coupling. If the stau is heavier than the smuon, we show that the bound can be as large as 1.4 (1.9) TeV. Such non-universal slepton mass spectrum generically predicts too large LFV/CPV. We show that the models are expected to be probed by LHC/ILC and LFV/CPV complementarily in future.

==> chapters/Conclusion.tex <==
%!TEX root = ../Dthesis.tex

\section{Conclusion}

Supersymmetry is one of most motivated candidate of new physics.
If the muon $g-2$ anomaly is solved by SUSY, some of superparticles are relatively light.
In this dissertation, we concentrated on the "minimal" SUSY model in which 
only the Bino and the slepton are light, while the other superparticles are decoupled.
In this model, the muon $g-2$ discrepancy is explained by the Bino-smuon diagram.
It is enhanced by large left-right mixing $m^2_{\widetilde{\ell }_{LR}}$.
We have investigated various phenomenologies in the minimal model.

The analyses were categorized by the slepton mass spectrum. 
When the mass spectrum is universal among the flavors, 
We found that the vacuum stability of the stau-Higgs potential restricts the smuon masses tightly. 
They are predicted to be within 330 (460) $\GeV$ at the $1\sigma$ ($2\sigma$) level of the muon $g-2$. 
It was shown that part of the parameter region is already excluded by LHC, 
and argued that such sleptons are expected to be studied at LHC or ILC in future.

If the staus are (much) heavier than the smuons, the vacuum stability bound of the staus is relaxed. 
In this mass spectrum, the smuon masses are limited by the vacuum stability condition of the smuon-Higgs potential. 
It was found that they are less than 1.4 (1.9) $\TeV$ at the $1\sigma$ ($2\sigma$)  level of the muon g − 2. 
Such slepton masses exceed the LHC/ILC reach. 
Instead, the non-universal slepton mass spectrum generically predicts too large LFV and EDM. 
They originate in the non-diagonal SM Yukawa matrices in the model basis. 
Although the prediction depends on the flavor models, LFV and/or EDM is very likely to be sizable in wide models. 
If no sleptons are discovered at LHC nor ILC, the model is expected to be probed by LFV and EDM sensitively.

In the universal mass spectrum case, the stau constribution to the Higgs coupling to di-photon $\kappa _{\gamma }$ might be also large.
The coupling will be measured at the percent levels by the joint analysis of HL-LHC and ILC.
Combining the information with that of the muon $g-2$, we may detect effects of the non-colored superparticles more definitely.
In this dissertation, we considered a situation that an excess of  $\kappa _{\gamma }$ is measured in HL-LHC and ILC.
First, we studied the stau mass region by using the vacuum meta-stability condition.
Consequently, we showed that the lightest stau $m_{\widetilde{\tau } _1}$ is predicted to be lighter than about 200\GeV, 
if the excess is measured to be larger than 4\% 
in the early stage of $\sqrt{s} = 500\GeV$ ILC.
Further, it was found that $m_{\widetilde{\tau } _1}$ is limited to be less than 290--460\GeV, if the excess is measured to be 1--2\% 
by accumulating luminosity at $\sqrt{s} =1\TeV$ ILC.
Such stau is within the kinematical reach of ILC.
Therefore, we concluded that the stau contribution to $\kappa _{\gamma }$ can be probed by discovering the stau, 
if the excess is measured in the future experiments, and if it originates in the stau contribution.

Once the stau is discovered at ILC, its properties are determined precisely. 
In this dissertation, we also studied the reconstruction of the stau contribution to $\kappa _{\gamma }$ by using the information which is available at ILC. 
It was estimated that the contribution can be reconstructed at $\sim 0.5\%$ at the sample point, which is comparable to or smaller than the measured value of the Higgs coupling. 
Thus, it is possible to test directly whether the excess originates in the stau contribution. 
Here, the measurement of the stau mixing angle is crucial. We also argued that, 
if the stau mixing angle is measured at the early stage of ILC, 
it is also possible to predict the heaviest stau mass, even when the heaviest stau is not yet discovered at the moment. 
Therefore, the stau contribution to $\kappa _{\gamma }$ can be probed not only by discovering the lightest stau, but also by studying the stau properties.

%Discoveries of new physics are the next target after the discovery of the Higgs boson. 
%The measurement of the Higgs couplings to di-photon is one of the hopeful channels to search for the new physics. 
%The stau contribution to the Higgs coupling could be probed or tested in future colliders by following the analysis in this letter.

\section{Discussion}

\TODO{stability : quantum correction}
\TODO{14 LHC, ILC, collider simulation -> sensitivity }
\TODO{Model Building}
\TODO{Cosmology}
\TODO{Other scenarios}

In conclusion, we studied the minimal SUSY models that explain the muon g − 2 discrepancy with the Bino-smuon contributions. 
It was shown that they are expected to be probed by LHC/ILC and LFV/EDM complementarily in future.





==> sections/current_mssm.tex <==
%!TEX root = ../Dthesis.tex


